Generative AI in Industrial Machine Vision -- A Review

Machine vision enhances automation, quality control, and operational efficiency in industrial applications by enabling machines to interpret and act on visual data. While traditional computer vision algorithms and approaches remain widely utilized, machine learning has become pivotal in current research activities. In particular, generative AI demonstrates promising potential by improving pattern recognition capabilities, through data augmentation, increasing image resolution, and identifying anomalies for quality control. However, the application of generative AI in machine vision is still in its early stages due to challenges in data diversity, computational requirements, and the necessity for robust validation methods. A comprehensive literature review is essential to understand the current state of generative AI in industrial machine vision, focusing on recent advancements, applications, and research trends. Thus, a literature review based on the PRISMA guidelines was conducted, analyzing over 1,200 papers on generative AI in industrial machine vision. Our findings reveal various patterns in current research, with the primary use of generative AI being data augmentation, for machine vision tasks such as classification and object detection. Furthermore, we gather a collection of application challenges together with data requirements to enable a successful application of generative AI in industrial machine vision. This overview aims to provide researchers with insights into the different areas and applications within current research, highlighting significant advancements and identifying opportunities for future work.

==> 07_conclusion.tex <==
\section{Conclusion}
% Summarize the main findings, contributions, limitations, and potential future research directions.

Although GenAI emerged as a new research field for industrial machine vision, focusing on generating synthetic data, enhancing pattern recognition, and more, there was a lack of literature reviews addressing the various approaches and subfields within the research community. A PRISMA literature review was conducted to analyze GenAI for industrial machine vision to answer research questions about the GenAI architectures used, their requirements and properties in this domain, as well as successfully applied applications. The main findings indicate the dominant use of GANs and VAEs as architectures, challenges related to the variety or shortage of images, and diverse applications across different industrial fields such as automotive and electronics. These findings suggest strong research activity around GenAI in industrial machine vision, with several subareas differing in architectures, specific requirements, and application fields in various industries. However, the findings are limited to the selected search string and the specific PRISMA procedure. While using different keywords might uncover additional literature and research methods, this article provides a robust foundation for exploring literature in GenAI for industrial Machine Vision and future literature research approaches as the field continues to evolve.
